Self-regulation of high-redshift black hole accretion via jets: challenges for SMBH formation

The early growth of black holes (BHs) in atomic-cooling halos is likely influenced by feedback on the surrounding gas. While the effects of radiative feedback are well-documented, mechanical feedback, particularly from AGN jets, has been comparatively less explored. Building on our previous work that examined the growth of a 100 ${M_\odot}$ BH in a constant density environment regulated by AGN jets, we expand the initial BH mass range from 1 to $10^4$ ${M_\odot}$ and adopt a more realistic density profile for atomic-cooling halos. We reaffirm the validity of our analytic models for jet cocoon propagation and feedback regulation. We identify several critical radii-namely, the terminal radius of jet cocoon propagation, the isotropization radius of the jet cocoon, and the core radius of the atomic-cooling halo-that are crucial in determining BH growth given specific gas properties and jet feedback parameters. In a significant portion of the parameter space, our findings show that jet feedback substantially disrupts the halo's core during the initial feedback episode, preventing BH growth beyond $10^4$ ${M_\odot}$. Conversely, conditions characterized by low jet velocities and high gas densities enable sustained BH growth over extended periods. We provide a prediction for the black hole mass growth as a function of time and feedback parameters. We found that, to form a supermassive BH ($>10^6 {M_\odot}$) within 1 Gyr entirely by accreting gas from an atomic-cooling halo, the jet energy feedback efficiency must be $\lesssim 10^{-4} \dot{M}_{BH} c^2$ even if the seed BH mass is $10^4 {M_\odot}$.

==> commented.tex <==
%Assuming $\alpha=1.05$ and $\xi=0.9$, we have
%$R^{1.4}\propto n_{\rm 0, Bondi}^{-0.64}$, pretty weak dependence again.

%This roughly agree with why we see the maximum propagation radii for the first blast wave is roughly the same across different density.
\begin{comment}
\subsection{Compared the numerics to the simulations}

Take the run for $n_{\rm 0 Bondi} =1e4{\rm cm}^{-3}$ for instance, from previous scaling $n_{\rm 0 c} \sim1\times10^3{\rm cm}^{-3}$, $\dot{M}_{0,J}\sim 3\times10^{-5} {\rm M_\odot} {\rm yr}^{-1}$. So
${E}_{\rm max, J}\sim 3\times10^{51} \rm{erg}$, $E_{\rm cool} (t)\sim 3.8\times10^{24} R^{\frac{2\alpha+2.1}{3}} \rm{erg}$.
In the end, $R\sim 19$ pc, roughly make sense.


\subsection{Integrated jet energy flux}
Assuming $n_{\rm 0, Bondi}$ is the initial density $n$ at Bondi Radii $r_{\rm Bondi}$. After the cocoon propagates beyond $r_{\rm Bondi}$, it already isotropizes in most cases. If not, it also quickly isotropizes after the density decreases.

From our previous paper \citep{2023MNRAS.520.4258S}, we have the energy conservation equations for the jet cocoon as it propagates in the bubble phase. Given the density evolution within the Bondi radius, the gas density is also a function of time.
\begin{align}
4\pi R^2 \rho_c(t) V_{\rm R Hot}^3 =\frac{\gamma }{2} \dot{M}_{\rm jet}(t) V_J^2\notag\\
V_{\rm R Hot}^2 \rho_c(t)=V_R^2 \rho_{\rm  Bondi}(t).
\end{align}

Supposed $\dot{M}_{\rm Jet} (t)\propto n_{\rm Bondi}^\alpha (t)$, where $\alpha\sim\frac{3-\xi}{2}$ for isotropic case, and $n_c (t)\propto n_{\rm Bondi}^\xi(t)$, and $\xi \lesssim 1$.

We now have density profile goes as $r^{-2}$: 
\begin{align}
\rho_{\rm Bondi}(t)=\rho_{\rm 0, Bondi}\left(\frac{R(t)}{r_{\rm Bondi}}\right)^{-2} \notag\\
\rho_{\rm c}(t)=\rho_{\rm 0, c}\left(\frac{R(t)}{r_{\rm Bondi}}\right)^{-2},
\end{align}
so
\begin{align}
\dot{M}_{\rm Jet}(t)=\dot{M}_{\rm 0, Jet} \left(\frac{n(t)}{n_{\rm 0,Bondi}}\right)^\alpha=\dot{M}_{\rm 0, Jet} \left(\frac{R(t)}{r_{\rm Bondi}}\right)^{-2 \alpha}.
\end{align}
Putting (1-3) together, we get:
\begin{align}
V_R=\left(\frac{\gamma}{8\pi}\right)^{1/3} \dot{M}_{0, J}^{1/3}V_J^{2/3} \rho_{0,c}^{1/6} \rho_{\rm 0,Bondi}^{-1/2}r_{\rm Bondi}^{\frac{-2+2\alpha}{3}}R^{-2\alpha/3}.
\end{align}

So the net jet energy is 
\begin{align}
{E}_{\rm tot, J}(t) =&\int \frac{1}{2} \dot{M}_J V_J^2 dt\notag\\
                        =&\int \frac{1}{2} \dot{M}_{0, J} \left(\frac{R}{r_{\rm Bondi}}\right)^{-2 \alpha} V_J^2 V_R^{-1} dR\notag\\
                        =&\left(\frac{\gamma}{\pi}\right)^{-1/3}\dot{M}_{0,J}^{2/3}r_{\rm Bondi}^{\frac{2+4\alpha}{3}} V_J^{4/3} \rho_{0,c}^{1/6} \rho_{\rm 0, Bondi}^{1/2} \notag\\
                        &\left(\frac{3}{4\alpha-3}\right)\left(r_{\rm Bondi}^{\frac{3-4\alpha}{3}} -R^{\frac{3-4\alpha}{3}} \right).
\end{align}

This saturates to a maximum value.
\begin{align}
{E}_{\rm max, J} &=\left(\frac{\gamma}{\pi}\right)^{-1/3}\dot{M}_{0,J}^{2/3}r_{\rm Bondi}^{\frac{5}{3}} V_J^{4/3} \rho_{0,c}^{1/6} \rho_{\rm 0, Bondi}^{1/2} \left(\frac{3}{4\alpha-3}\right)\notag\\
&\propto n_{\rm 0, Bondi}^{\frac{2\alpha}{3}-\frac{\xi}{6}+\frac{1}{2}}
\end{align}
For $\alpha=1.5$ from measurement, $\xi=0.9$ from measurement, we have ${E}_{\rm max, J}\propto n_{\rm 0, Bondi}^{1.35}$.

For $\alpha=1.05$ from toy model from $\xi$, $\xi=0.9$ from measurement, we have ${E}_{\rm max, J}\propto n_{\rm 0, Bondi}^{1.05}$.


\subsection{The integrated cocoon cooling}
The instant cooling rate within the jet cocoon at a specific time is:
\begin{align}
\dot{E}_{\rm Cool} (t) &=\int\limits^R_0\Lambda 4\pi r^2 dr\notag\\
                        &\sim {\bf C} \frac{4\pi}{3} n_c^2 R^3 \left(\frac{T}{10^6}\right)^{-0.7}\notag\\
                        &\sim {\bf C} \frac{4\pi}{3} n_{\rm 0, c}^2 \left(\frac{R}{r_{\rm Bondi}}\right)^{-4} R^3 \left(\frac{T}{10^6}\right)^{-0.7}
\end{align}

To estimate the temperature, we have:
\begin{align}
\frac{3}{2}n_c kT \frac{4}{3}\pi R^3\sim E_{\rm max}\notag\\
T\sim \frac{E_{\rm max}}{2\pi k r_{\rm Bondi}^2 n_{\rm 0 ,c}} \frac{1}{R}\sim T_0 \left(\frac{R}{r_{\rm Bondi}}\right)^{-1},
\end{align}
where $T_0\sim \frac{E_{\rm max}}{2\pi k r_{\rm Bondi}^3 n_{\rm 0 ,c}}$.

So
\begin{align}
\dot{E}_{\rm Cool} (t)\sim\frac{4\pi}{3} {\bf C} n_{\rm 0 c}^2 \left(\frac{T_0}{10^6}\right)^{-0.7} r_{\rm Bondi}^{3.3} R^{-0.3}.
\end{align}

The accumulated cooling up to the time the bubble reaches $R$ would then be:
\begin{align}
E_{\rm cool} (t)=&\int \dot{E}_{\rm cool}  dt=\int \dot{E}_{\rm cool} V^{-1} dR\notag\\
                =&\frac{4\pi}{3} {\bf C} n_{\rm 0,c}^2 \left(\frac{T_0}{10^6}\right)^{-0.7} r_{\rm Bondi}^{3.3+\frac{-2\alpha+2}{3}} \left(\frac{\gamma}{8\pi}\right)^{-1/3}\dot{M}_{0,J}^{-1/3}\notag\\
                & V_J^{-2/3} \rho_{0,c}^{-1/6}\rho_{\rm 0,Bondi}^{1/2}\left(\frac{3}{2\alpha+2.1}\right)\left(R^{\frac{2\alpha+2.1}{3}}-R_{\rm iso}^{\frac{2\alpha+2.1}{3}}\right)\notag\\
                \propto & n_{\rm 0 c} ^{2.7-1/6} n_{\rm 0 Bondi} ^{1/2-\alpha/3} E_{\rm max}^{-0.7} R^{\frac{2\alpha+2.1}{3}}
\end{align}

\subsection{The terminal Radius}
Assuming $E_{\rm cool} (t)\sim E_{\rm max, J} (t)$ and solve for $R$, for $\alpha=1.5$ and $\xi=0.9$, we have
$R^{1.7}\propto n_{\rm 0, Bondi}^{0.015}$, super weak dependence as we see.

Assuming $\alpha=1.05$ and $\xi=0.9$, we have
$R^{1.4}\propto n_{\rm 0, Bondi}^{-0.64}$, pretty weak dependence again.

This roughly agrees with why we see the maximum propagation radii for the first blast wave is roughly the same across different densities.

\subsection{Compared the numerics to the simulations}

Take the run for $n_{\rm 0 Bondi} =1e4{\rm cm}^{-3}$ for instance, from previous scaling $n_{\rm 0 c} \sim1\times10^3{\rm cm}^{-3}$, $\dot{M}_{0,J}\sim 3\times10^{-5} {\rm M_\odot} {\rm yr}^{-1}$. So
${E}_{\rm max, J}\sim 3\times10^{51} \rm{erg}$, $E_{\rm cool} (t)\sim 3.8\times10^{24} R^{\frac{2\alpha+2.1}{3}} \rm{erg}$.
In the end, $R\sim 19$ pc, roughly make sense.
\end{comment}
